LogiCoT: Logical Chain-of-Thought Instruction-Tuning

Generative Pre-trained Transformer 4 (GPT-4) demonstrates impressive chain-of-thought reasoning ability. Recent work on self-instruction tuning, such as Alpaca, has focused on enhancing the general proficiency of models. These instructions enable the model to achieve performance comparable to GPT-3.5 on general tasks like open-domain text generation and paraphrasing. However, they fall short of helping the model handle complex reasoning tasks. To bridge the gap, this paper presents LogiCoT, a new instruction-tuning dataset for Logical Chain-of-Thought reasoning with GPT-4. We elaborate on the process of harvesting instructions for prompting GPT-4 to generate chain-of-thought rationales. LogiCoT serves as an instruction set for teaching models of logical reasoning and elicits general reasoning skills.

==> Table/code.tex <==
\begin{algorithmic}[1]
\State prompt\_with\_cot\{

    `instruction': instruction,
    %``instruction'': ``Translate the following inference to logic notation'',

    `input': input,
    %``input'': `` It is windy if and only if it is sunny \textbackslash n Mary is not driving a car\textbackslash n Mary is driving a car if and only if it is windy\textbackslash n Therefore it is not sunny or Susan is a soldier\textbackslash n'',

    `output': output,
    %``outpu'': ``p $\leftrightarrow$ q\textbackslash n ¬r\textbackslash n r $\leftrightarrow$ p\textbackslash n Therefore ¬q or s\textbackslash n'',
    
    \}

\State prompt\_without\_cot\{

    `instruction': instruction,
    %``instruction'': ``You will be presented with a passage and a question about that passage. There are four options to be chosen from, you need to choose the only correct option to answer that question. If the first option is right, you generate the answer `A', if the second option is right, you generate the answer `B', if the third option is right, you generate the answer `C', if the fourth option is right, you generate the answer `D'. Read the question and options thoroughly and select the correct answer from the four answer labels. Read the passage thoroughly to ensure you know what the passage entails.'',

    `input': input,
    %``input'': `` Passage: Altogether, the students in Ms. Tarnowski' s Milton Elementary School class collected more aluminum cans than did the students in any of the school' s other classes. Ttherefore, the Milton student who collected the most aluminum cans was in Ms. Tarnowski' s class.\textbackslash n Question: Which one of the following arguments contains flawed reasoning that is most parallel to that in the argument above?\textbackslash nA. Mr. Rowe's Milton Elementary School class raised more money by selling candy bars than Ms. Hunt's class raised by holding a raffle. Ttherefore, the number of candy bars sold by Mr. Rowe's class was greater than the number of raffle tickets sold by Ms. Hunt's class.\textbackslash nB. More than half of Milton Elementary School's students play in the band and more than half of the school's students sing in the choir. Ttherefore, every student at Milton Elementary School either plays in the band or sings in the choir.\textbackslash nC. The total number of tickets to the school fair sold by the students in Ms. Ramirez's Milton Elementary School class was greater than the number sold by Milton students from any other class. Ttherefore, the Milton student who sold the most tickets to the school fair was a student in Ms. Ramirez's class.\textbackslash nD. Ms. Ventura's Milton Elementary School class assembled more birdhouses than did any of the school's other classes. Since Ms. Ventura's class had fewer students than any other Milton class, her students assembled more birdhouses, on average, than did the students in any other Milton class.\textbackslash nAnswer and reasoning step by step'',
    
    %``output'': ``C. The total number of tickets to the school fair sold by the students in Ms. Ramirez's Milton Elementary School class was greater than the number sold by Milton students from any other class. Therefore, the Milton student who sold the most tickets to the school fair was a student in Ms. Ramirez's class.\textbackslash n Reasoning: In both the original argument and option C, the premise is that one class as a whole outperformed other classes in a collection-type activity (aluminum cans or tickets sold). They conclude that the top individual performer in that activity must have come from the class that collected the most, which is flawed reasoning because it does not take into account individual contributions within each class.''
    
    \}
    
\State output = openai.ChatCompletion.create(
    
    model = "gpt-4",
    
    messages = [\{`role': `system', `content': instruction\}, \{`role': `user', `content': input\}, \{`role': `assistant', `content': cot\}]
    
    )
\end{algorithmic}

==> Table/mmlu_bak.tex <==
\begin{table}
\centering
\scalebox{0.75}{
\begin{tabular}{l|c|c|c}
\hline
\multirow{2}{}{\textbf{Task}} & \multicolumn{2}{c|}{\textbf{LLaMA-7b}} & \textbf{ChatGPT} \\

 & \textbf{base} & \textbf{logicot} & \\
\hline
Math & 25.1 & \textbf{29.0} & \\
Health & 34.0 & \textbf{42.9} & \\
Physics & 29.4 & \textbf{34.2} & \\
Business & 34.8 & \textbf{57.2} & \\
Biology & 32.4 & \textbf{46.5} & \\
Chemistry & 25.4 & \textbf{33.0} & \\
Computer science & 28.2 & \textbf{40.0} \\
Economics & 26.5 & \textbf{38.5} \\
Engineering & 25.5 & \textbf{32.4} \\
Philosophy & 30.8 & \textbf{37.6}\\
Other & 40.4 & \textbf{50.8} \\
History & 38.2 & \textbf{55.2} \\
Geography & 28.8 & \textbf{52.5} \\
Politics & 32.1 & \textbf{53.4} \\
Psychology & 33.2 & \textbf{50.9} \\
Culture & 37.3 & \textbf{56.9}\\
Law & 29.3 & \textbf{39.6} \\
STEM & 27.6 & \textbf{34.8} \\
Humanities & 31.6 & \textbf{41.8} \\
Social Sciences & 31.5 & \textbf{49.2} \\
Other (misc.) & 36.4 & \textbf{47.7} \\
\hline
Average & 31.8 & \textbf{43.3} \\
\hline
\end{tabular}
}
\caption{\label{Tab:mmlu}
MMLU results. All results are in \%, the best results are in \textbf{bold}.
}
\end{table}

